Three Things to Know about Deep Metric Learning

This paper addresses supervised deep metric learning for open-set image retrieval, focusing on three key aspects: the loss function, mixup regularization, and model initialization. In deep metric learning, optimizing the retrieval evaluation metric, recall@k, via gradient descent is desirable but challenging due to its non-differentiable nature. To overcome this, we propose a differentiable surrogate loss that is computed on large batches, nearly equivalent to the entire training set. This computationally intensive process is made feasible through an implementation that bypasses the GPU memory limitations. Additionally, we introduce an efficient mixup regularization technique that operates on pairwise scalar similarities, effectively increasing the batch size even further. The training process is further enhanced by initializing the vision encoder using foundational models, which are pre-trained on large-scale datasets. Through a systematic study of these components, we demonstrate that their synergy enables large models to nearly solve popular benchmarks.

==> data_ab_temp.tex <==
\pgfplotstableread{
 		temp	sop_r1		cars_r1    sop_simix_r1     cars_simix_r1
 		0.1		81.00	76.7	81.41       86.79
 		0.5		82.67	80.6	81.83       86.42
 		1.0		82.83	80.8	82.13       88.17
 		2.0		82.80	80.6	82.15       86.15
 		5.0		82.43	80.3	82.00       86.66
 	}{\yfccLambda}


==> tab_cars196.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{ll|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  & r@1   & r@2 &  r@4  & r@8 \\
    	\hline\hline
    	
	ProxyNCA \cite{mtl+17} & $I_{1}^{128}$ &
	$73.2$ &
	$82.4$ &
	$86.4$ &
	$88.7$ 
	\\
	
	Margin \cite{wms+17} & $R_{50}^{128}$ &
	$\underline{79.6}$ &
	$\underline{86.5}$ &
	$\underline{91.9}$ &
	$\underline{95.1}$ 
	\\
	
	\hline
	RS@k\textsuperscript{\dag} & $R_{50}^{128}$ &
	$78.1$  &
	$85.8$  &
	$91.1$  &
	$94.5$ 
    \\

	RS@k\textsuperscript{\dag} (+log) & $R_{50}^{128}$ &
	$78.9$  &
	$86.7$  &
	$91.8$  &
	$95.0$ 
    \\
    
    %& &
    %\tiny{\textcolor{red}{$-7.4\%$}} &
    %\tiny{\textcolor{red}{$-5.2\%$}} &
    %\tiny{\textcolor{red}{$-9.9\%$}} &
	%\tiny{\textcolor{red}{$-12\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{128}$ &
	\bm{$84.7$}  &
	\bm{$90.9$}  &
	\bm{$94.7$}  &
	\bm{$96.9$} 
	\\

	RS@k\textsuperscript{\dag} (+log +SiMix) &
	$R_{50}^{128}$ &
	$83.5$ &
	$90.4$ &
	$94.4$ &
	$96.8$
	\\
	
	%& & 
	%\tiny{\textcolor{blue}{$+25\%$}} &
	%\tiny{\textcolor{blue}{$+33\%$}} &
	%\tiny{\textcolor{blue}{$+35\%$}} &
	%\tiny{\textcolor{blue}{$+37\%$}}
	%\\
	
	\hline \hline
	MS \cite{whh+19} & $I_{3}^{512}$ &
	$84.1$ &
	$90.4$ &
	$94.0$ &
	$96.1$ 
	\\
	
	
	NormSoftMax \cite{zw18} & $R_{50}^{512}$ &
	$84.2$ &
	$90.4$ &
	$94.4$ &
	$96.9$
    \\
	
	HORDE \cite{jph+19} & $I_{3}^{512}$ &
	$86.2$ &
	$91.9$ &
	$95.1$ &
	$97.2$
	\\
	
	ProxyNCA++ \cite{tdt20} & $R_{50}^{512}$ &
	$\underline{86.5}$ &
	$\underline{92.5}$ &
	$\underline{95.7}$ &
	\bm{$\underline{97.7}$}
	\\
	
	SAP\textsuperscript{\dag} \cite{bxk+20} & $R_{50}^{512}$ &
	$76.1$ &
	$84.3$ &
	$89.8$ &
	$93.8$ 
	\\
	
	SAP\textsuperscript{\dag} \cite{bxk+20} (+GeM +LN)  & $R_{50}^{512}$ &
	$78.2$ &
	$85.6$ &
	$90.8$ &
	$94.3$ 
	\\
	
	\hline
	SAP++\textsuperscript{\dag} & $R_{50}^{512}$ &
	$79.5$ &
	$86.6$ &
	$91.2$ &
	$94.4$ 
	\\
	
	SAP++\textsuperscript{\dag} (+SiMix) & $R_{50}^{512}$ &
	$85.4$ &
	$91.0$ &
	$94.3$ &
	$96.7$ 
	\\
	
	\hline 
	RS@k\textsuperscript{\dag} &  $R_{50}^{512}$ &
	$80.8$ &
	$88.1$ & 
	$92.2$ &
	$95.3$
	\\

	RS@k\textsuperscript{\dag} (+log) & $R_{50}^{512}$ &
	$80.9$  &
	$88.1$  &
	$92.5$  &
	$95.7$ 
    \\
	
	%& & 
	%\tiny{\textcolor{red}{$-42\%$}} &
	%\tiny{\textcolor{red}{$-58\%$}} &
	%\tiny{\textcolor{red}{$-81\%$}} &
	%\tiny{\textcolor{red}{$-104\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{512}$ &
	$87.3$ &
	$92.6$ & 
	$95.7$ &
	$97.4$ 
	\\

	RS@k\textsuperscript{\dag} (+log +SiMix) & $R_{50}^{512}$ &
	$88.0$ &
	$93.1$ & 
	\bm{$96.3$} &
	\bm{$98.0$} 
	\\
	
	RS@k\textsuperscript{\dag} (+SiMix bs=588) & $R_{50}^{512}$ &
	\bm{$88.3$} &
	\bm{$93.3$} & 
	$95.9$ &
	$97.6$ 
	\\
	
	%& & 
	%\tiny{\textcolor{blue}{$+13\%$}} &
	%\tiny{\textcolor{blue}{$+11\%$}} &
	%\tiny{\textcolor{blue}{$+4.7\%$}} &
	%\tiny{\textcolor{red}{$-4.3\%$}} 
	%\\
	\hline
    \end{tabular}

==> tab_cars196_ab_temp.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  r@1   & r@2 &  r@4  & r@8 & r@16 & Avg\\
    	\hline\hline
    	
        RS@k\textsuperscript{\dag} $\tau_{1}=0.1$ &
        $76.7$ &
        $84.3$ &
        $89.8$ &
        $93.4$ &
        $96.1$ &
        $88.1$
        \\
        
        RS@k\textsuperscript{\dag} $\tau_{1}=0.5$ &
        $80.6$ &
        $87.5$ &
        $92.2$ &
        $95.2$ &
        $97.3$ &
        $90.5$
        \\
	
	    RS@k\textsuperscript{\dag} $\tau_{1}=1.0$ &
        $80.8$ &
        $87.6$ &
        $92.2$ &
        $95.0$ &
        $97.1$ &
        $90.5$
        \\
        
        RS@k\textsuperscript{\dag} $\tau_{1}=2.0$ &
        $80.6$ &
        $87.6$ &
        $92.1$ &
        $95.0$ &
        $97.1$ &
        $90.5$
        \\
        
        RS@k\textsuperscript{\dag} $\tau_{1}=5.0$ &
        $80.3$ &
        $87.4$ &
        $92.0$ &
        $95.2$ &
        $97.2$ &
        $90.4$
        \\
       \hline
       \multicolumn{6}{c}{with SiMix} \\
       \hline
        RS@k\textsuperscript{\dag} $\tau_{1}=0.1$ &
        $86.79$ &
        $92.74$ &
        $95.71$ &
        $97.56$ &
        $98.89$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=0.5$ &
        $86.66$ &
        $92.03$ &
        $95.03$ &
        $97.40$ &
        $98.73$
        \\

	    RS@k\textsuperscript{\dag}  $\tau_{1}=1.0$ &        $88.17$ &
        $93.01$ &
        $95.92$ &
        $97.42$ &
        $98.66$
        \\

        RS@k\textsuperscript{\dag}  $\tau_{1}=2.0$ &
        $86.15$ &
        $91.50$ &
        $94.81$ &
        $97.04$ &
        $98.54$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=5.0$ &
        $86.42$ &
        $91.91$ &
        $95.35$ &
        $97.29$ &
        $98.60$
        \\
        
	\hline
    \end{tabular}

==> tab_cars196_bs.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  r@1   & r@2 &  r@4  & r@8 & r@16 &Avg\\
    	\hline\hline
    	
        RS@k\textsuperscript{\dag} (bs$=16$) &
        $74.60$ &
        $83.18$ &
        $89.44$ &
        $93.69$ &
        $96.11$
        \\


        RS@k\textsuperscript{\dag} (bs$=32$) &
        $77.04$ &
        $85.13$ &
        $90.21$ &
        $93.92$ &
        $96.54$
        \\

        RS@k\textsuperscript{\dag} (bs$=64$) &
        $76.67$ &
        $84.95$ &
        $90.22$ &
        $94.44$ &
        $96.90$
        \\

        RS@k\textsuperscript{\dag} (bs$=128$) &
        $78.92$ &
        $86.31$ &
        $91.46$ &
        $94.79$ &
        $96.81$
        \\

        RS@k\textsuperscript{\dag} (bs$=256$) &
        $79.14$ &
        $86.73$ &
        $91.64$ &
        $95.08$ &
        $97.18$
        \\

        RS@k\textsuperscript{\dag} (bs$=392$) &
        $80.72$ &
        $88.34$ &
        $92.79$ &
        $95.70$ &
        $97.58$
        \\
        
     \hline 
     \multicolumn{7}{c}{with SiMix}  \\
     \hline
        RS@k\textsuperscript{\dag} (bs$=16$) &
        $86.27$ &
        $91.94$ &
        $95.35$ &
        $97.31$ &
        $98.61$
        \\

        RS@k\textsuperscript{\dag} (bs$=32$) &
        $87.46$ &
        $92.68$ &
        $95.86$ &
        $97.75$ &
        $98.78$
        \\

        RS@k\textsuperscript{\dag} (bs$=64$) &
        $87.31$ &
        $92.23$ &
        $95.60$ &
        $97.40$ &
        $98.68$
        \\

        RS@k\textsuperscript{\dag} (bs$=128$) &
        $87.43$ &
        $92.82$ &
        $95.67$ &
        $97.81$ &
        $98.73$
        \\

        RS@k\textsuperscript{\dag} (bs$=256$) &
        $87.06$ &
        $92.46$ &
        $95.63$ &
        $97.28$ &
        $98.56$
        \\

        RS@k\textsuperscript{\dag} (bs$=392$) &
        $88.17$ &
        $93.01$ &
        $95.92$ &
        $97.42$ &
        $98.66$
        \\

	\hline
    \end{tabular}

==> tab_inat.tex <==
\setlength\extrarowheight{-2pt}
    \begin{tabular}{ll|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  & r@1   & r@4 &  r@16  & r@32\\
    	\hline\hline
    	
	Margin \cite{wms+17} & $R_{50}^{128}$ &
	$58.1$ & 
	$75.5$ & 
	$86.8$ & 
	$\underline{90.7}$
	\\
	
	ProxyNCA \cite{mtl+17} & $R_{50}^{128}$ &
	$\underline{61.6}$ & 
	$\underline{77.4}$ & 
	$\underline{87.0}$ & 
	$90.6$
	\\
	
	\hline
	RS@k\textsuperscript{\dag} & $R_{50}^{128}$ &
	${69.3}$  &
	${82.9}$  &
	${90.6}$  &
	${93.1}$ 
	\\

	RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{128}$ &
	$70.0$ &
	$83.6$ &
	$91.2$ &
	$93.6$
	\\
	
	%& & 
	%\tiny{\textcolor{blue}{$+20\%$}} &
	%\tiny{\textcolor{blue}{$+24\%$}} &
	%\tiny{\textcolor{blue}{$+28\%$}} &
	%\tiny{ \textcolor{blue}{$+27\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{128}$ &
	\bm{$69.6$}  & 
	\bm{$83.3$}  & 
	\bm{$91.2$}  & 
	\bm{$93.8$}
	\\
	
	& & 
	\tiny{\textcolor{blue}{$+21\%$}} &
	\tiny{\textcolor{blue}{$+26\%$}} &
	\tiny{\textcolor{blue}{$+32\%$}} &
	\tiny{\textcolor{blue}{$+34\%$}}
	\\

	RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{128}$ &
	  & 
	  &
	  &
	
	\\
	
	\hline \hline
	FastAP \cite{chx+19} & $R_{50}^{512}$ &
	$60.6$ & 
	$77.0$ & 
	$87.2$ & 
	$90.6$
	\\
	
	Blackbox AP \cite{rmp+20} & $R_{50}^{512}$ &
	$62.9$ &
	$79.0$ &
	$88.9$ &
	$92.1$
	\\
	
	SAP \cite{bxk+20} & $R_{50}^{512}$ &
	$\underline{67.2}$ &
	$\underline{81.8}$ &
	$\underline{90.3}$ &
	$\underline{93.1}$
	\\
	
	SAP\textsuperscript{\dag} \cite{bxk+20} (+GeM +LN) & $R_{50}^{512}$ &
	$68.7$ &
	$82.7$ &
	$90.9$ &
	$93.5$ 
	\\
	
	\hline
	RS@k\textsuperscript{\dag} & $R_{50}^{512}$ &
	${71.2}$ &
	${84.0}$ &
	${91.3}$ &
	${93.6}$
	\\

	RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{512}$ &
	$71.7$ &
	$84.4$ &
	$91.6$ &
	$94.0$
	\\
	
    	%& & 
	%\tiny{\textcolor{blue}{$+12.0\%$}} &
	%\tiny{\textcolor{blue}{$+12\%$}} &
	%\tiny{\textcolor{blue}{$+10\%$}} &
	%\tiny{\textcolor{blue}{$+7.2\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix)& $R_{50}^{512}$ &
	\bm{$71.8$}  &
	\bm{$84.7$}  &
	\bm{$91.9$}  &
	\bm{$94.3$}
	\\
	
	& & 
	\tiny{\textcolor{blue}{$+14\%$}} &
	\tiny{\textcolor{blue}{$+16\%$}} &
	\tiny{\textcolor{blue}{$+16\%$}} &
	\tiny{\textcolor{blue}{$+17\%$}}
	\\

	RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{512}$ &
	  & 
	  &
	  &
	
	\\
	
    %\hline\hline
    
    %SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B$_{32}^{512}$ &
	%$72.2$ &
	%$84.6$ &
	%$91.6$ &
	%$93.9$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{32}^{512}$ & 
    %$75.9$ & 
    %$87.1$ &
    %$93.1$ &
    %$95.1$
    %\\
	
	%SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B$_{16}^{512}$ &
	%$79.1$ &
	%$89.0$ &
	%$94.2$ &
	%$95.8$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{16}^{512}$ & 
    %$83.9$ & 
    %$92.1$ &
    %$95.9$ &
    %$97.2$
    %\\
	
	\hline
    \end{tabular}

==> tab_metriclearning_initialization_gappa.tex <==
\begin{tabular}{lll|cccc}
\hline
 \multirow{2}[1]{*}{Init.} & \multirow{2}[1]{*}{Arch.$^\text{dim}$} & \multirow{2}[1]{*}{Method}  & \multicolumn{4}{c}{GAPPA} \\
& & & \multicolumn{4}{c}{recall@k} \\
& & & $1$ & $10^1$ & $10^2$ & $10^3$  \\
\hline

\multirow{6}[3]{*}{IN-21K} & \multirow{2}[1]{*}{ViT-B/$32^{512}$}  & SAP & 
$79.1$ & 
$93.2$ & 
$98.0$ & 
$99.6$ 
\\

&  & RS@k &
$81.8$ & 
$94.8$ & 
$98.5$ & 
$99.7$

\\

& \multirow{2}[1]{*}{ViT-B/$16^{512}$} & SAP & 
$84.1$ & 
$95.2$ & 
$98.6$ & 
$99.7$
\\

&  & RS@k &
$86.6$ & 
$96.4$ & 
$98.9$ & 
$\underline{99.8}$
\\

& \multirow{2}[1]{*}{ViT-L/$16^{512}$} & SAP &
$85.7$ & 
$95.6$ & 
$98.6$ & 
$99.7$ 
\\

&  & RS@k & 
$88.3$ & 
$96.8$ & 
$99.0$ & 
$\underline{99.8}$
\\

\hline

% Results with CLIP LAION-400M Init.
\multirow{6}[3]{*}{CLIP-400M} & \multirow{2}[1]{*}{ViT-B/$32^{512}$}  & SAP & 
$77.4$ & 
$92.3$ & 
$97.7$ & 
$99.5$ 
\\

& &  RS@k & 
$79.8$ & 
$94.0$ & 
$98.3$ & 
$99.6$ 
\\

& \multirow{2}[1]{*}{ViT-B/$16^{512}$} & SAP & 
$82.9$ & 
$94.7$ & 
$98.5$ & 
$99.7$ 
\\

&  & RS@k &
$86.7$ & 
$96.4$ & 
$99.0$ & 
$\underline{99.8}$ 
\\

& \multirow{2}[1]{*}{ViT-L/$14^{512}$} & SAP &
$86.5$ & 
$95.9$ & 
$98.8$ & 
$\underline{99.8}$
\\

&  & RS@k & 
$89.6$ & 
$97.3$ & 
$99.2$ & 
$\bm{99.9}$ 
\\

\hline

% Results with CLIP LAION-2B Init.
\multirow{6}[3]{*}{CLIP-2B} & \multirow{2}[1]{*}{ViT-B/$32^{512}$}  & SAP & 
$78.4$ & 
$93.0$ & 
$98.0$ & 
$99.6$ 
\\

& &  RS@k & 
$81.1$ & 
$94.5$ & 
$98.6$ & 
$\underline{99.8}$ 
\\

& \multirow{2}[1]{*}{ViT-B/$16^{512}$} & SAP & 
$83.5$ & 
$95.0$ & 
$98.6$ & 
$99.7$ 
\\

&  & RS@k &
$87.7$ & 
$96.7$ & 
$99.1$ & 
$\underline{99.8}$ 
\\

& \multirow{2}[1]{*}{ViT-L/$14^{512}$} & SAP &
$87.2$ & 
$96.3$ & 
$98.9$ & 
$\underline{99.8}$ 
\\

&  & RS@k & 
$90.5$ & 
$97.7$ & 
$\bm{99.4}$ & 
$\bm{99.9}$ 
\\

\hline

% Results with  DiHT Init.
\multirow{6}[3]{*}{DiHT} & \multirow{2}[1]{*}{ViT-B/$32^{512}$}  & SAP & 
$80.0$ & 
$93.4$ & 
$98.0$ & 
$99.6$ 
\\

& &  RS@k & 
$83.2$ & 
$95.2$ & 
$98.7$ & 
$\underline{99.8}$
\\

& \multirow{2}[1]{*}{ViT-B/$16^{512}$} & SAP & 
$85.0$ & 
$95.4$ & 
$98.7$ & 
$\underline{99.8}$ 
\\

&  & RS@k &
$88.8$ & 
$97.0$ & 
$99.2$ & 
$\underline{99.8}$ 
\\

& \multirow{2}[1]{*}{ViT-L/$14^{512}$} & SAP &
$88.8$ & 
$96.7$ & 
$99.0$ & 
$\underline{99.8}$ 
\\

&  & RS@k & 
$\underline{91.6}$ & 
$\bm{97.9}$ & 
$\bm{99.4}$ & 
$\bm{99.9}$ 
\\

\hline

% Results with  SWAG Init.
\multirow{4}[2]{*}{SWAG} & \multirow{2}[1]{*}{ViT-B/$16^{512}$} & SAP & 
$85.0$ & 
$95.0$ & 
$98.4$ & 
$99.7$ 
\\

&  & RS@k &
$88.8$ & 
$96.8$ & 
$99.0$ & 
$\underline{99.8}$ 
\\

& \multirow{2}[1]{*}{ViT-L/$16^{512}$} & SAP &
$87.6$ & 
$96.0$ & 
$98.7$ & 
$\underline{99.8}$ 
\\

&  & RS@k & 
$90.9$ & 
$97.5$ & 
$99.2$ & 
$\underline{99.8}$ 
\\

\hline

% Results with DINOv2 Init.
\multirow{2}[1]{*}{DINOv2} & \multirow{2}[1]{*}{ViT-L/$14^{512}$} & SAP &
$89.1$ & 
$96.6$ & 
$98.9$ & 
$\underline{99.8}$ 
\\

&  & RS@k & 
$\bm{91.8}$ & 
$\underline{97.8}$ & 
$\underline{99.3}$ & 
$\underline{99.8}$
\\

\hline

\end{tabular}


==> tab_metriclearning_sota.tex <==
\begin{tabular}{l|l|l|l}
\hline
 Dataset & Our best results & Previous state-of-the-art & \% error reduction \\
\hline

iNaturalist & $90.0$ & $83.9$ Patel {\em et al.} 2022 & \textcolor{blue}{$+37.9\%$} \\
SOP & $90.8$ & $88.0$ Patel {\em et al.} 2022 & \textcolor{blue}{$+17.4\%$} \\
Cars196 & $97.2$ & $94.8$ Jun {\em et al.} 2019 & \textcolor{blue}{$+46.2\%$} \\
CUB200 & $90.2$ & $85.6$ Ermolov {\em et al.} 2022 & \textcolor{blue}{$+31.9\%$} \\

\hline

\end{tabular}


==> tab_sop.tex <==
\setlength\extrarowheight{-2pt}
    \begin{tabular}{ll|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  & r@$10^{0}$   & r@$10^{1}$ &  r@$10^{2}$  & r@$10^{3}$\\
    	\hline\hline
	ProxyNCA \cite{mtl+17} & $I_{1}^{128}$ &
	$73.7$ & 
	- & 
	- & 
	- 
	\\
	
	Margin \cite{wms+17} & $R_{50}^{128}$ &
	$72.7$ &
	$86.2$ & 
	$93.8$ & 
	$98.0$
	\\
	
	Divide \cite{skp+15} & $R_{50}^{128}$ &
	$75.9$ & 
	$88.4$ & 
	$94.9$ &
	$98.1$
	\\
	
	MIC \cite{rbo+19} & $R_{50}^{128}$ &
	$77.2$ &
	$89.4$ &
	$95.6$ &
	- 
	\\
	
	Cont. w/M \cite{wzh+20} & $R_{50}^{128}$ &
	$\underline{80.6}$ &
	$\underline{91.6}$ &
	$\underline{96.2}$ &
	$\underline{98.7}$
	\\
	
	\hline
	RS@k\textsuperscript{\dag} & $R_{50}^{128}$ &
	$80.6$ &
	$91.6$ &
	$96.4$ &
	\bm{$98.8$} 
	\\

	RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{128}$ &
	$81.2$ & 
	$91.9$ & 
	$96.5$ & 
    $98.8$
	\\
	
	%& & 
	%\tiny{\textcolor{red}{$\pm 0.0\%$}} &
	%\tiny{\textcolor{red}{$\pm 0.0\%$}} &
	%\tiny{\textcolor{blue}{$+5.3\%$}} &
	%\tiny{\textcolor{blue}{$+7.7\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{128}$ &
	\bm{$80.9$} &
	\bm{$91.7$} &
	\bm{$96.5$} &
	\bm{$98.8$}
	\\
	
	& & 
	\tiny{\textcolor{blue}{$+1.5\%$}} &
	\tiny{\textcolor{blue}{$+1.2\%$}} &
	\tiny{\textcolor{blue}{$+7.9\%$}} &
	\tiny{\textcolor{blue}{$+7.7\%$}}
	\\

	RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{128}$ &
	  & 
	  &
	  &
	
	\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{32}^{512}$ & 
    %$83.3$ & 
    %$93.6$ &
    %$97.6$ &
    %$99.3$
    %\\
    
    %RS@k\textsuperscript{\dag} & ViT-B$_{16}^{512}$ & 
    %$86.5$ & 
    %$95.2$ &
    %$98.2$ &
    %$99.4$
    %\\

    \hline \hline
	FastAP \cite{chx+19} & $R_{50}^{512}$ &
	$76.4$ &
	$89.0$ & 
	$95.1$ & 
	$98.2$ 
	\\
	
	MS \cite{whh+19} & $I_{3}^{512}$ &
	$78.2$ &
	$90.5$ &
	$96.0$ &
	$98.7$
	\\
	
	NormSoftMax \cite{zw18} & $R_{50}^{512}$ &
	$78.2$ &
	$90.6$ &
	$96.2$ &
	- 
	\\
	
	Blackbox AP \cite{rmp+20} & $R_{50}^{512}$ &
	$78.6$ &
	$90.5$ &
	$96.0$ &
	$98.7$
	\\
	
	Cont. w/M \cite{wzh+20} & $I_{3}^{512}$ &
	$79.5$ &
	$90.8$ &
	$96.1$ &
	$98.7$
	\\
	
	HORDE \cite{jph+19} & $R_{50}^{512}$ &
	$80.1$ &
	$91.3$ &
	$96.2$ &
	- 
	\\
	
	ProxyNCA++ \cite{tdt20} & $R_{50}^{512}$ &
	$\underline{80.7}$ &
	$\underline{92.5}$ &
	$96.7$ &
	$98.9$
	\\
	
	SAP \cite{bxk+20} & $R_{50}^{512}$ &
	$80.1$ &
	$91.5$ &
	$\underline{96.6}$ & 
	$\underline{99.0}$
	\\
	
	SAP\textsuperscript{\dag} \cite{bxk+20} (+GeM +LN) & $R_{50}^{512}$ &
	$80.3$ &
	$92.0$ &
	$96.9$ &
	$99.0$
	\\

	\hline
	RS@k\textsuperscript{\dag} (bs=384) & $R_{50}^{512}$ &
	$81.2$ & 
	$92.2$ & 
	$96.9$ & 
	$99.0$ 
	\\
	
	%& & 
	%\tiny{\textcolor{blue}{$+2.6\%$}} &
	%\tiny{\textcolor{red}{$-4.0\%$}} &
	%\tiny{\textcolor{red}{$+8.8\%$}} &
	%\tiny{\textcolor{red}{$\pm0.0\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} & $R_{50}^{512}$ &
	\bm{$82.7$}  & 
	\bm{$92.8$} & 
	\bm{$97.0$} & 
	$99.0$ 
	\\

	RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{512}$ &
	$83.0$ & 
	$93.0$ & 
	$97.1$ & 
    $99.0$
	\\
	
	%& & 
	%\tiny{\textcolor{blue}{$+10\%$}} &
	%\tiny{\textcolor{blue}{$+4.0\%$}} &
	%\tiny{\textcolor{blue}{$+12\%$}} &
	%\tiny{\textcolor{red}{$\pm 0.0\%$}} &
	%\\
	
	RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{512}$ &
	${82.1}$  & 
	\bm{$92.8$}  &
	\bm{$97.0$}  &
	\bm{$99.1$}
	\\
	
	& & 
	\tiny{\textcolor{blue}{$+7.3\%$}} &
	\tiny{\textcolor{blue}{$+4.0\%$}} &
	\tiny{\textcolor{blue}{$+12\%$}} &
	\tiny{\textcolor{blue}{$+10\%$}}
	\\

	RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{512}$ &
	  & 
	  &
	  &
	
	\\

    %\hline\hline
    
    %SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B$_{32}^{512}$ &
	%$83.7$ &
	%$94.0$ &
	%$97.8$ &
	%$99.3$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{32}^{512}$ & 
    %$85.1$ & 
    %$94.6$ &
    %$98.0$ &
    %$99.3$
    %\\
	
	%SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B$_{16}^{512}$ &
	%$86.6$ &
	%$95.4$ &
	%$98.4$ &
	%$99.5$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{16}^{512}$ & 
    %$88.0$ & 
    %$96.1$ &
    %$98.6$ &
    %$99.6$
    %\\

	\hline    	
    \end{tabular}

==> tab_sop_ab.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{l|c|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  R@$10^{0}$   & R@$10^{1}$ &  R@$10^{2}$  & R@$10^{3}$ & Avg\\
    	\hline\hline
    	
        SR@$\{1\}$\textsuperscript{\dag} &
        $82.8$ &
        $92.6$ &
        $96.8$ &
        $98.8$ &
        $92.8$
        \\
        
        SR@$\{1,2\}$\textsuperscript{\dag} &
        $82.8$ &
        $92.7$ &
        $96.8$ &
        $98.9$ &
        $92.8$
        \\
	
	    SR@$\{1,2,4\}$\textsuperscript{\dag} &
        $83.0$ &
        $92.9$ &
        $96.9$ &
        $98.9$ &
        $92.9$
        \\
        
        SR@$\{1,2,4,8\}$\textsuperscript{\dag} &
        $82.7$ &
        $92.8$ &
        $97.0$ &
        $98.9$ &
        $92.9$
        \\
        
        SR@$\{1,2,4,8,16\}$\textsuperscript{\dag} &
        $82.7$ &
        $92.8$ &
        $97.0$ &
        $99.0$ &
        $92.9$
        \\
	\hline
    \end{tabular}

==> tab_sop_bs.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{l|c|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  r@$10^{0}$   & r@$10^{1}$ &  r@$10^{2}$  & r@$10^{3}$ & Avg\\
    	\hline\hline
    	
        RS@k\textsuperscript{\dag} (bs$=16$) &
        $72.9$ &
        $85.9$ &
        $93.5$ &
        $97.9$ &
        $87.6$
        \\


        RS@k\textsuperscript{\dag} (bs$=32$) &
        $77.3$ &
        $89.5$ &
        $95.7$ &
        $98.8$ &
        $90.3$
        \\

        RS@k\textsuperscript{\dag} (bs$=64$) &
        $79.0$ &
        $90.8$ &
        $96.4$ &
        $99.0$ &
        $91.3$
        \\

        RS@k\textsuperscript{\dag} (bs$=128$) &
        $79.7$ &
        $91.1$ &
        $96.4$ &
        $99.0$ &
        $91.5$
        \\

        RS@k\textsuperscript{\dag} (bs$=256$) &
        $80.5$ &
        $91.7$ &
        $96.7$ &
        $99.0$ &
        $92.0$
        \\

        RS@k\textsuperscript{\dag} (bs$=512$) &
        $81.2$ &
        $92.2$ &
        $96.9$ &
        $99.0$ &
        $92.3$
        \\

        RS@k\textsuperscript{\dag} (bs$=1024$) &
        $82.0$ &
        $92.6$ &
        $97.0$ &
        $99.0$ &
        $92.7$
        \\

        RS@k\textsuperscript{\dag} (bs$=2048$) &
        $82.5$ &
        $92.9$ &
        $97.1$ &
        $99.1$ &
        $92.8$
        \\

        RS@k\textsuperscript{\dag} (bs$=4096$) &
        $82.8$ &
        $92.9$ &
        $97.1$ &
        $99.1$ &
        $92.9$
        \\
     \hline 
     \multicolumn{6}{c}{with SiMix}  \\
     \hline
        RS@k\textsuperscript{\dag} (bs$=16$) &
        \\


        RS@k\textsuperscript{\dag} (bs$=32$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=64$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=128$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=256$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=512$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=1024$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=2048$) &
        \\

        RS@k\textsuperscript{\dag} (bs$=4096$) &
        \\
	\hline
    \end{tabular}

==> tab_sop_temp.tex <==
\setlength\extrarowheight{-2pt}
   \begin{tabular}{l|c|c|c|c|c}
    \hline
    \multicolumn{1}{l}{Method} &  r@$10^{0}$   & r@$10^{1}$ &  r@$10^{2}$  & r@$10^{3}$ & Avg\\
    	\hline\hline
    	
        RS@k\textsuperscript{\dag} $\tau_{1}=0.1$ &
        $81.00$ &
        $91.54$ &
        $96.22$ &
        $98.74$
        \\
        
        RS@k\textsuperscript{\dag} $\tau_{1}=0.5$ &
        $82.67$ &
        $92.85$ &
        $96.97$ &
        $98.98$
        \\

	    RS@k\textsuperscript{\dag} $\tau_{1}=1.0$ &
	    $82.83$ &
	    $92.90$ &
	    $96.96$ &
	    $98.96$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=2.0$ &
        $82.80$ &
        $92.95$ &
        $97.05$ &
        $98.98$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=5.0$ &
        $82.43$ &
        $97.78$ &
        $97.00$ &
        $99.03$
        \\
        
       \hline
       \multicolumn{6}{c}{with SiMix} \\
       \hline
        RS@k\textsuperscript{\dag} $\tau_{1}=0.1$ &
        $81.41$ &
        $92.29$ &
        $96.77$ &
        $98.90$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=0.5$ &
        $81.83$ &
        $92.53$ &
        $96.83$ &
        $98.92$
        \\

	    RS@k\textsuperscript{\dag}  $\tau_{1}=1.0$ &
	    $82.13$ &
	    $92.80$ &
	    $97.00$ &
	    $99.10$
        \\

        RS@k\textsuperscript{\dag}  $\tau_{1}=2.0$ &
        $82.15$ &
        $92.66$ &
        $96.87$ &
        $98.93$
        \\

        RS@k\textsuperscript{\dag} $\tau_{1}=5.0$ &
        $82.00$ &
        $92.60$ &
        $96.84$ &
        $98.93$
        \\
       
	\hline
    \end{tabular}

==> tab_vid.tex <==
\setlength\extrarowheight{-2pt}
    \begin{tabular}{ll|cc|cc|cc}
    \hline
    \multicolumn{1}{l}{\multirow{2}[2]{*}{Method}}
          && \multicolumn{2}{c|}{Small} & \multicolumn{2}{c|}{Medium} & \multicolumn{2}{c}{Large} \\
          && r@1   & r@5   & r@1   &  r@5   & r@1   & r@5 \\ \hline \hline
    Divide \cite{skp+15} & $R_{50}^{128}$ &
    $87.7$ &
    $92.9$ &
    $85.7$ &
    $90.4$ &
    $82.9$ &
    $90.2$
    \\
    
    MIC \cite{rbo+19} & $R_{50}^{128}$ &
    $86.9$ &
    $93.4$ &
    - &
    - &
    $82.0$ &
    $91.0$
    \\
    
    Cont. w/M \cite{wzh+20} & $R_{50}^{128}$ &
    $\underline{94.7}$ &
    $\underline{96.8}$ &
    $\underline{93.7}$ &
    $\underline{95.8}$ &
    $\underline{93.0}$ &
    $\underline{95.8}$
    \\
    
    \hline
    RS@k\textsuperscript{\dag} & $R_{50}^{128}$ &
    \bm{$95.6$} &
    \bm{$97.8$} &
    \bm{$94.4$} &
    \bm{$96.8$} &
    \bm{$93.5$} &
    \bm{$96.6$}
    \\

    & & 
    \tiny{\textcolor{blue}{$+17\%$}} & 
    \tiny{\textcolor{blue}{$+31\%$}} &
    \tiny{\textcolor{blue}{$+11\%$}} &
    \tiny{\textcolor{blue}{$+24\%$}} &
    \tiny{\textcolor{blue}{$+7.1\%$}} &
    \tiny{\textcolor{blue}{$+19\%$}}
    \\

    RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{128}$ &
    $95.7$ &
    $97.8$ &
    $94.5$ &
    $96.9$ &
    $93.8$ &
    $96.7$
    \\
    
    
    RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{512}$ &
    $95.4$ &
    $97.5$ &
    $93.8$ &
    $96.6$ &
    $93.0$ &
    $96.2$
    \\

    RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{128}$ &
     &
     &
     &
     &
     &
    
    \\
    
    \hline \hline
    
    FastAP \cite{chx+19} & $R_{50}^{512}$ &
    $91.9$ &
    $96.8$ &
    $90.6$ &
    $95.9$ &
    $87.5$ &
    $95.1$
    \\
    
    Cont. w/M \cite{wzh+20} & $I_{3}^{512}$ &
    $94.6$ &
    $96.9$ &
    $\underline{93.4}$ &
    $96.0$ &
    $\underline{93.0}$ &
    $96.1$
    \\
    
    SAP \cite{bxk+20} & $R_{50}^{512}$ &
    $\underline{94.9}$ &
    $\underline{97.6}$ &
    $93.3$ &
    $\underline{96.4}$ &
    $91.9$ &
    $\underline{96.2}$
    \\
    
    
    SAP\textsuperscript{\dag} \cite{bxk+20} (+GeM +LN) & $R_{50}^{512}$ &
    $94.2$ &
    $97.2$ &
    $92.7$ &
    $96.2$ &
    $91.0$ &
    $95.8$
    \\
    \hline
    
    RS@k\textsuperscript{\dag} & $R_{50}^{512}$ &
    \bm{$95.7$} &
    \bm{$97.9$} &
    \bm{$94.6$} &
    \bm{$96.9$} &
    \bm{$93.8$} &
    \bm{$96.6$}
    \\
    
    & & 
    \tiny{\textcolor{blue}{$+16\%$}} & 
    \tiny{\textcolor{blue}{$+13\%$}} &
    \tiny{\textcolor{blue}{$+18\%$}} &
    \tiny{\textcolor{blue}{$+13\%$}} &
    \tiny{\textcolor{blue}{$+11\%$}} &
    \tiny{\textcolor{blue}{$+11\%$}}
    \\

    RS@k\textsuperscript{\dag} (+log-rank) & $R_{50}^{512}$ &
    $95.9$ &
    $97.9$ &
    $94.7$ &
    $97.1$ &
    $94.1$ &
    $97.0$   
    \\


    
    RS@k\textsuperscript{\dag} (+SiMix) & $R_{50}^{512}$ &
    $95.3$ &
    $97.7$ &
    $94.2$ &
    $96.5$ &
    $93.3$ &
    $96.4$
    \\

    RS@k\textsuperscript{\dag} (+log-rank +SiMix) & $R_{50}^{512}$ &
     &
     &
     &
     &
     &
    
    \\

    %\hline\hline
    
    %SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B$_{32}^{512}$ &
	%$94.8$ &
	%$97.7$ &
	%$93.5$ &
	%$96.8$ &
	%$92.1$ &
	%$96.3$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{32}^{512}$ & 
    %$95.1$ & 
    %$97.7$ &
    %$94.1$ &
    %$96.7$ &
    %$93.2$ &
    %$96.5$
    %\\
	
    %SAP\textsuperscript{\dag} %\cite{bxk+20} & ViT-B$_{16}^{512}$ &
	%$95.5$ &
	%$97.7$ &
	%$94.2$ &
	%$96.9$ &
	%$93.1$ &
	%$96.6$
	%\\

    %RS@k\textsuperscript{\dag} & ViT-B$_{16}^{512}$ & 
    %$96.2$ & 
    %$98.0$ &
    %$95.2$ &
    %$97.2$ &
    %$94.7$ &
    %$97.1$
    %\\
    
    \hline
    \end{tabular}

==> tab_vit.tex <==
\setlength\extrarowheight{-2pt}
    \begin{tabular}{ll|c|c|c|c|c|c|c|c|cc|cc|cc|c|c|c|c}
    \hline
    \multirow{3}[1]{*}{Method}& \multirow{3}[1]{*}{Arch.} & \multicolumn{4}{c|}{Inaturalist} & \multicolumn{4}{c|}{SOP} & \multicolumn{6}{c|}{VehicleID} &
    \multicolumn{4}{c}{CARS196}\\
    \cline{3-20}
    & & & & & & & & & & \multicolumn{2}{c|}{Small} & \multicolumn{2}{c|}{Medium} & \multicolumn{2}{c|}{Large} \\
    & & r@1 & r@4 & r@16 & r@32 & r@$10^0$ & r@$10^1$ & r@$10^2$ & r@$10^3$ & r@1 & r@5 & r@1 & r@5 & r@1 & r@5 & r@1 & r@2 & r@4 & r@8\\
    \hline \hline

    
    SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B/32 &
    $72.2$ &
	$84.6$ &
	$91.6$ &
	$93.9$ &
	
    $83.7$ &
	$94.0$ &
	$97.8$ &
	$99.3$ &
	
	$94.8$ &
	$97.7$ &
	$93.5$ &
	$96.8$ &
	$92.1$ &
	$96.3$
	\\

    RS@k\textsuperscript{\dag} & ViT-B/32 & 
    $75.9$ & 
    $87.1$ &
    $93.1$ &
    $95.1$ &

    $85.1$ & 
    $94.6$ &
    $98.0$ &
    $99.3$ &

    $95.1$ & 
    $97.7$ &
    $94.1$ &
    $96.7$ &
    $93.2$ &
    $96.5$
    \\

    RS@k\textsuperscript{\dag} (+log-rank) & ViT-B/32 & 
    & 
    &
    &
    &

    $85.2$ &
    $94.7$ &
    $98.1$ &
    $99.4$ &

    &
    &
    &
    &
    &
    \\
	
    SAP\textsuperscript{\dag} \cite{bxk+20} & ViT-B/16 &
	$79.1$ &
	$89.0$ &
	$94.2$ &
	$95.8$ &
	
	$86.6$ &
	$95.4$ &
	$98.4$ &
	$99.5$ &

	$95.5$ &
	$97.7$ &
	$94.2$ &
	$96.9$ &
	$93.1$ &
	$96.6$
	\\

    RS@k\textsuperscript{\dag} & ViT-B/16 & 
    $83.9$ & 
    $92.1$ &
    $95.9$ &
    $97.2$ &
    
    $88.0$ & 
    $96.1$ &
    $98.6$ &
    $99.6$ &
    
    $96.2$ & 
    $98.0$ &
    $95.2$ &
    $97.2$ &
    $94.7$ &
    $97.1$
    \\

    RS@k\textsuperscript{\dag} (+log-rank) & ViT-B/16 & 
    & 
    &
    &
    &

    $88.2$ &
    $96.4$ &
    $98.6$ &
    $99.6$ &

    &
    &
    &
    &
    &
    \\
    
    \hline
    \end{tabular}
